AI-based Drone Assisted Human Rescue in Disaster Environments: Challenges and Opportunities

In this survey we are focusing on utilizing drone-based systems for the detection of individuals, particularly by identifying human screams and other distress signals. This study has significant relevance in post-disaster scenarios, including events such as earthquakes, hurricanes, military conflicts, wildfires, and more. These drones are capable of hovering over disaster-stricken areas that may be challenging for rescue teams to access directly. Unmanned aerial vehicles (UAVs), commonly referred to as drones, are frequently deployed for search-and-rescue missions during disaster situations. Typically, drones capture aerial images to assess structural damage and identify the extent of the disaster. They also employ thermal imaging technology to detect body heat signatures, which can help locate individuals. In some cases, larger drones are used to deliver essential supplies to people stranded in isolated disaster-stricken areas. In our discussions, we delve into the unique challenges associated with locating humans through aerial acoustics. The auditory system must distinguish between human cries and sounds that occur naturally, such as animal calls and wind. Additionally, it should be capable of recognizing distinct patterns related to signals like shouting, clapping, or other ways in which people attempt to signal rescue teams. To tackle this challenge, one solution involves harnessing artificial intelligence (AI) to analyze sound frequencies and identify common audio signatures. Deep learning-based networks, such as convolutional neural networks (CNNs), can be trained using these signatures to filter out noise generated by drone motors and other environmental factors. Furthermore, employing signal processing techniques like the direction of arrival (DOA) based on microphone array signals can enhance the precision of tracking the source of human noises.

==> nomenclature.tex <==


\newlength\myitemwidth
\setlength\myitemwidth{5em} % <<< choose what you need here
\newlist{myacronymlist}{description}{1}
\setlist[myacronymlist]{
  labelindent = 0pt ,
  labelsep    = 0pt ,
  leftmargin  = \myitemwidth ,
  labelwidth  = \myitemwidth ,
  itemindent  = 0pt ,
  format      = \normalfont
}

\usepackage{acro}
\DeclareAcroListStyle{myliststyle}{list}{
  list = myacronymlist
}
\acsetup{ list-style = myliststyle }

\DeclareAcronym{IoT}{
  short = \normalfont{IoT} ,
  long  = Internet-of-Things,
  sort  = i,
  class = nomencl
}
\DeclareAcronym{4G}{
  short = \normalfont{4G} ,
  long  =  The fourth generation,
  sort  = 4,
  class = nomencl
}
\DeclareAcronym{5G}{
  short = \normalfont{5G} ,
  long  =  The fifth generation,
  sort  = 5,
  class = nomencl
}

\DeclareAcronym{6G}{
  short = \normalfont{6G} ,
  long  =  The sixth generation,
  sort  = 6,
  class = nomencl
}

\DeclareAcronym{LDS}{
  short = \normalfont{LDS} ,
  long  =  Low-density spreading,
  sort  = lds,
  class = nomencl
}

\DeclareAcronym{NOMA}{
  short = \normalfont{NOMA} ,
  long  =  Non-orthogonal multiple access,
  sort  = noma,
  class = nomencl
}

\DeclareAcronym{MPA}{
  short = \normalfont{MPA} ,
  long  =  Message passing algorithm,
  sort  = mpa,
  class = nomencl
}

\DeclareAcronym{MAP}{
  short = \normalfont{MAP} ,
  long  = Maximum a posteriori detector,
  sort  = map,
  class = nomencl
}

\DeclareAcronym{MMSE}{
  short = \normalfont{MMSE} ,
  long  = Minimum mean-square estimation,
  sort  = mmse,
  class = nomencl
}

\DeclareAcronym{BER}{
  short = \normalfont{BER} ,
  long  = Bit-error-rate,
  sort  = ber,
  class = nomencl
}

\DeclareAcronym{MUD}{
  short = \normalfont{MUD} ,
  long  = Multiuser detection,
  sort  = mud,
  class = nomencl
}


\DeclareAcronym{MIMO}{
  short = \normalfont{MIMO} ,
  long  = Multiple-input multiple-output,
  sort  = mimo,
  class = nomencl
}

\DeclareAcronym{M2M}{
  short = \normalfont{M2M} ,
  long  = Machine-to-machine,
  sort  = m2m,
  class = nomencl
}

\DeclareAcronym{D2D}{
  short = \normalfont{D2D} ,
  long  = Device-to-device,
  sort  = d2d,
  class = nomencl
}

\DeclareAcronym{D2E}{
  short = \normalfont{D2E} ,
  long  = Device-to-everything ,
  sort  = d2e,
  class = nomencl
}

\DeclareAcronym{IoV}{
  short = \normalfont{IoV} ,
  long  = Internet of Vehicles,
  sort  = iov,
  class = nomencl
}

\DeclareAcronym{MTC}{
  short = \normalfont{MTC} ,
  long  = Machine-type communication,
  sort  = mtc,
  class = nomencl
}

\DeclareAcronym{ITS}{
  short = \normalfont{ITS} ,
  long  = Intelligent transportation system,
  sort  = its,
  class = nomencl
}

\DeclareAcronym{OMA}{
  short = \normalfont{OMA} ,
  long  = Orthogonal multiple access,
  sort  = oma,
  class = nomencl
}

\DeclareAcronym{TDMA}{
  short = \normalfont{TDMA} ,
  long  = Time-division multiple access,
  sort  = tdma,
  class = nomencl
}

\DeclareAcronym{FDMA}{
  short = \normalfont{FDMA} ,
  long  = Frequency division multiple access,
  sort  = fdma,
  class = nomencl
}

\DeclareAcronym{CDMA}{
  short = \normalfont{CDMA} ,
  long  = Code-division multiple access,
  sort  = cdma,
  class = nomencl
}


\DeclareAcronym{SCMA}{
  short = \normalfont{SCMA} ,
  long  = Sparse code multiple access,
  sort  = scma,
  class = nomencl
}

\DeclareAcronym{PDMA}{
  short = \normalfont{PDMA} ,
  long  = Pattern division multiple access,
  sort  = pdma,
  class = nomencl
}

\DeclareAcronym{MUSA}{
  short = \normalfont{MUSA} ,
  long  = Multiuser shared access,
  sort  = musa,
  class = nomencl
}

\DeclareAcronym{MMTC}{
  short = \normalfont{mMTC} ,
  long  = Massive machine-type-communications,
  sort  = mmtc,
  class = nomencl
}


\DeclareAcronym{LDPC}{
  short = \normalfont{LDPC} ,
  long  = Low-density parity-check,
  sort  = ldpc,
  class = nomencl
}


\DeclareAcronym{AWGN}{
  short = \normalfont{AWGN} ,
  long  = Additive white Gaussian noise,
  sort  = awgn,
  class = nomencl
}

\DeclareAcronym{FIR}{
  short = \normalfont{FIR} ,
  long  = Finite impulse response,
  sort  = fir,
  class = nomencl
}

\DeclareAcronym{CIR}{
  short = \normalfont{CIR} ,
  long  = Channel impulse response,
  sort  = cir,
  class = nomencl
}

\DeclareAcronym{MF}{
  short = \normalfont{MF} ,
  long  = Matched filter,
  sort  = mf,
  class = nomencl
}

\DeclareAcronym{ZF}{
  short = \normalfont{ZF} ,
  long  = Zero-forcing filter,
  sort  = zf,
  class = nomencl
}

\DeclareAcronym{SIC}{
  short = \normalfont{SIC} ,
  long  = Successive interference cancellation,
  sort  = sic,
  class = nomencl
}

\DeclareAcronym{PIC}{
  short = \normalfont{PIC} ,
  long  = Parallel interference cancellation,
  sort  = pic,
  class = nomencl
}

\DeclareAcronym{PDA}{
  short = \normalfont{PDA} ,
  long  = Probabilistic data association,
  sort  = pda,
  class = nomencl
}

\DeclareAcronym{BP}{
  short = \normalfont{BP} ,
  long  = Believe propagation,
  sort  = bp,
  class = nomencl
}

\DeclareAcronym{JSG}{
  short = \normalfont{JSG} ,
  long  = Joint sparse graph ,
  sort  = jsg,
  class = nomencl
}

\DeclareAcronym{BPSK}{
  short = \normalfont{BPSK} ,
  long  = Binary phase-shift keying  ,
  sort  = bpsk,
  class = nomencl
}

\DeclareAcronym{QPSK}{
  short = \normalfont{QPSK} ,
  long  = Quadrature phase-shift keying  ,
  sort  = qpsk,
  class = nomencl
}

\DeclareAcronym{QAM}{
  short = \normalfont{QAM} ,
  long  = Quadrature amplitude modulation  ,
  sort  = qam,
  class = nomencl
}

\DeclareAcronym{APP}{
  short = \normalfont{APP} ,
  long  = A posteriori probability  ,
  sort  = app,
  class = nomencl
}

\DeclareAcronym{LLR}{
  short = \normalfont{LLR} ,
  long  = Log-likelihood ratio  ,
  sort  = llr,
  class = nomencl
}

\DeclareAcronym{DE}{
  short = \normalfont{DE} ,
  long  = Domain equalization  ,
  sort  = de,
  class = nomencl
}

\DeclareAcronym{DFT}{
  short = \normalfont{DFT} ,
  long  = Discrete Fourier transform  ,
  sort  = dft,
  class = nomencl
}

\DeclareAcronym{IDFT}{
  short = \normalfont{IDFT} ,
  long  = Inverse discrete Fourier transform  ,
  sort  = idft,
  class = nomencl
}

\DeclareAcronym{CP}{
  short = \normalfont{CP} ,
  long  = Cyclic prefix  ,
  sort  = cp,
  class = nomencl
}

\DeclareAcronym{MAI}{
  short = \normalfont{MAI} ,
  long  = Multiple-access interference  ,
  sort  = mai,
  class = nomencl
}

\DeclareAcronym{RE}{
  short = \normalfont{RE},
  long  = Resource element,
  sort  = re,
  class = nomencl
}

\iffalse
\DeclareAcronym{ML}{
  short = \normalfont{ML} ,
  long  = Maximum-likelihood,
  sort  = ml,
  class = nomencl
}
\fi
\DeclareAcronym{FDE}{
  short = \normalfont{FDE} ,
  long  = Frequency domain equalization,
  sort  = fde,
  class = nomencl
}

\DeclareAcronym{OFDM}{
  short = \normalfont{OFDM} ,
  long  = Orthogonal frequency-division multiplexing,
  sort  = ofdm,
  class = nomencl
}

\DeclareAcronym{UD}{
  short = \normalfont{UD} ,
  long  = Uniquely decodable,
  sort  = ud,
  class = nomencl
}

\DeclareAcronym{IrLDS}{
  short = \normalfont{IrLDS} ,
  long  = Irregular low-density spreading,
  sort  = irlds,
  class = nomencl
}

\DeclareAcronym{VA}{
  short = \normalfont{VA} ,
  long  = Viterbi algorithm,
  sort  = va,
  class = nomencl
}

\DeclareAcronym{SD}{
  short = \normalfont{SD} ,
  long  = Sphere-decoding algorithm,
  sort  = sd,
  class = nomencl
}

\DeclareAcronym{SISO}{
  short = \normalfont{SISO} ,
  long  = Soft-input soft-output,
  sort  = siso,
  class = nomencl
}

\DeclareAcronym{GML}{
  short = \normalfont{GML} ,
  long  = Global maximum likelihood detector,
  sort  = gml,
  class = nomencl
}

\DeclareAcronym{SNR}{
  short = \normalfont{SNR} ,
  long  = Signal-to-noise ratio,
  sort  = snr,
  class = nomencl
}

\DeclareAcronym{LRS}{
  short = \normalfont{LRS} ,
  long  = Large random spreading,
  sort  = lrs,
  class = nomencl
}

\DeclareAcronym{QLSS}{
  short = \normalfont{QLSS} ,
  long  = Quasi-large sparse sequence,
  sort  = qlss,
  class = nomencl
}

\DeclareAcronym{SER}{
  short = \normalfont{SER} ,
  long  = Symbol error rate,
  sort  = ser,
  class = nomencl
}

\DeclareAcronym{MC}{
  short = \normalfont{MC} ,
  long  = Multicarrier,
  sort  = mc,
  class = nomencl
}

\DeclareAcronym{JSFG}{
  short = \normalfont{JSFG} ,
  long  = Joint sparse factor graph,
  sort  = jsfg,
  class = nomencl
}

\DeclareAcronym{SMI}{
  short = \normalfont{SMI} ,
  long  = Single user mutual information,
  sort  = smi,
  class = nomencl
}

\DeclareAcronym{SVE}{
  short = \normalfont{SVE} ,
  long  = Spreading vector extension,
  sort  = sve,
  class = nomencl
}

\DeclareAcronym{LDSM}{
  short = \normalfont{LDSM} ,
  long  = Low-density superposition modulation,
  sort  = ldsm,
  class = nomencl
}

\DeclareAcronym{BBPSO}{
  short = \normalfont{BBPSO} ,
  long  = Bare-bone particle swarm optimization,
  sort  = bbpso,
  class = nomencl
}

\DeclareAcronym{STS}{
  short = \normalfont{STS} ,
  long  = Steiner triple system,
  sort  = sts,
  class = nomencl
}

\DeclareAcronym{BIBD}{
  short = \normalfont{BIBD} ,
  long  = Balanced incomplete block design,
  sort  = bibd,
  class = nomencl
}

\DeclareAcronym{LDSMA}{
  short = \normalfont{LDSMA} ,
  long  = Low-density spreading multiple access,
  sort  = ldsma,
  class = nomencl
}

\DeclareAcronym{GMAC}{
  short = \normalfont{GMAC} ,
  long  = Gaussian multiple access channel,
  sort  = gmac,
  class = nomencl
}

\DeclareAcronym{BLER}{
  short = \normalfont{BLER} ,
  long  = Block error rate,
  sort  = bler,
  class = nomencl
}

\DeclareAcronym{MAC}{
  short = \normalfont{MAC} ,
  long  = Multiple access channel,
  sort  = mac,
  class = nomencl
}

\DeclareAcronym{EXIT}{
  short = \normalfont{EXIT} ,
  long  = Extrinsic information transfer,
  sort  = exit,
  class = nomencl
}

\DeclareAcronym{SEP}{
  short = \normalfont{SEP} ,
  long  = Symbol error probability,
  sort  = sep,
  class = nomencl
}

\DeclareAcronym{MS}{
  short = \normalfont{MS} ,
  long  = Mobile station,
  sort  = ms,
  class = nomencl
}

\DeclareAcronym{SFBC}{
  short = \normalfont{SFBC} ,
  long  = Space-frequency block codes,
  sort  = sfbc,
  class = nomencl
}

\DeclareAcronym{SM}{
  short = \normalfont{SM} ,
  long  = Spatial modulation,
  sort  = sm,
  class = nomencl
}

\DeclareAcronym{SCDMA}{
  short = \normalfont{SCDMA} ,
  long  = Sparse code-division multiple-access,
  sort  = scdma,
  class = nomencl
}

\DeclareAcronym{FBMC}{
  short = \normalfont{FBMC} ,
  long  = Filter-bank multicarrier,
  sort  = fbmc,
  class = nomencl
}

\DeclareAcronym{LDWM}{
  short = \normalfont{LDWM} ,
  long  = Low-density weight matrix,
  sort  = ldwm,
  class = nomencl
}

\DeclareAcronym{ULDS}{
  short = \normalfont{ULDS} ,
  long  = Ultra low-density spread,
  sort  = ulds,
  class = nomencl
}

\DeclareAcronym{SSM}{
  short = \normalfont{SSM} ,
  long  = Sparse superposition matrix,
  sort  = ssm,
  class = nomencl
}

\DeclareAcronym{SINR}{
  short = \normalfont{SINR} ,
  long  = Signal-to-interference-noise ratio,
  sort  = sinr,
  class = nomencl
}

\DeclareAcronym{TSC}{
  short = \normalfont{TSC} ,
  long  = Total squared correlation,
  sort  = tsc,
  class = nomencl
}

\DeclareAcronym{WBE}{
  short = \normalfont{WBE} ,
  long  = Welch-bound-equality,
  sort  = wbe,
  class = nomencl
}

\DeclareAcronym{MWBE}{
  short = \normalfont{MWBE} ,
  long  = Maximum-Welch-bound-equality,
  sort  = mwbe,
  class = nomencl
}

\DeclareAcronym{CM}{
  short = \normalfont{CM} ,
  long  = Coded modulation,
  sort  = cm,
  class = nomencl
}

\DeclareAcronym{MLCM}{
  short = \normalfont{MLCM} ,
  long  = Multilevel coded modulation,
  sort  = mlcl,
  class = nomencl
}

\DeclareAcronym{TCM}{
  short = \normalfont{TCM} ,
  long  = Trellis-coded modulation,
  sort  = tcm,
  class = nomencl
}

\DeclareAcronym{TTCM}{
  short = \normalfont{TTCM} ,
  long  = Turbo trellis-coded modulation,
  sort  = ttcm,
  class = nomencl
}

\DeclareAcronym{ED}{
  short = \normalfont{ED} ,
  long  = Euclidean distance,
  sort  = ed,
  class = nomencl
}

\DeclareAcronym{BICM}{
  short = \normalfont{BICM} ,
  long  = Bit-interleaved coded modulation,
  sort  = bicm,
  class = nomencl
}

\DeclareAcronym{LTE}{
  short = \normalfont{LTE} ,
  long  = Long-term evolution,
  sort  = lte,
  class = nomencl
}

\DeclareAcronym{QPP}{
  short = \normalfont{QPP} ,
  long  = Quadratic permutation polynomial,
  sort  = qpp,
  class = nomencl
}

\DeclareAcronym{PEG}{
  short = \normalfont{PEG} ,
  long  = Progressive edge-growth,
  sort  = peg,
  class = nomencl
}

\DeclareAcronym{EMB}{
  short = \normalfont{EMB} ,
  long  = Enhanced mobile broadband,
  sort  = emb,
  class = nomencl
}

\DeclareAcronym{uRLLC}{
  short = \normalfont{uRLLC} ,
  long  = Ultra-reliable low-latency communications,
  sort  = urllc,
  class = nomencl
}

\DeclareAcronym{mmWave}{
  short = \normalfont{mmWave} ,
  long  = Millimeter-wave,
  sort  = mmwave,
  class = nomencl
}

\DeclareAcronym{AI}{
  short = \normalfont{AI} ,
  long  = Artificial intelligence,
  sort  = ai,
  class = nomencl
}

\DeclareAcronym{BS}{
  short = \normalfont{BS} ,
  long  = Base station,
  sort  = bs,
  class = nomencl
}

\DeclareAcronym{CNN}{
  short = \normalfont{CNN} ,
  long  = Convolutional neural network,
  sort  = cnn,
  class = nomencl
}

\DeclareAcronym{DNN}{
  short = \normalfont{DNN} ,
  long  = Deep neural network,
  sort  = dnn,
  class = nomencl
}

\DeclareAcronym{DQL}{
  short = \normalfont{DQL} ,
  long  = Deep Q-learning,
  sort  = dql,
  class = nomencl
}

\DeclareAcronym{DQN}{
  short = \normalfont{DQN} ,
  long  = Deep Q-network,
  sort  = dqn,
  class = nomencl
}

\DeclareAcronym{DRL}{
  short = \normalfont{DRL} ,
  long  = Deep reinforcement learning,
  sort  = drl,
  class = nomencl
}

\DeclareAcronym{ER}{
  short = \normalfont{ER} ,
  long  = Experience replay,
  sort  = er,
  class = nomencl
}

\DeclareAcronym{FMAP}{
  short = \normalfont{FMAP} ,
  long  = Flying mesh access point,
  sort  = fmap,
  class = nomencl
}

\DeclareAcronym{GPS}{
  short = \normalfont{GPS} ,
  long  = Global positioning system,
  sort  = gps,
  class = nomencl
}

\DeclareAcronym{LoS}{
  short = \normalfont{LoS} ,
  long  = Line-of-sight,
  sort  = los,
  class = nomencl
}

\DeclareAcronym{ML}{
  short = \normalfont{ML} ,
  long  = Machine learning,
  sort  = ml,
  class = nomencl
}
\DeclareAcronym{MDP}{
  short = \normalfont{MDP} ,
  long  = Markov decision process,
  sort  = mdp,
  class = nomencl
}
\DeclareAcronym{MOS}{
  short = \normalfont{MOS} ,
  long  = Mean opinion score,
  sort  = mop,
  class = nomencl
}
\DeclareAcronym{MINLP}{
  short = \normalfont{MINLP} ,
  long  = Mixed-integer non-linear problem,
  sort  = minlp,
  class = nomencl
}

\DeclareAcronym{NLoS}{
  short = \normalfont{NLoS} ,
  long  = No-line-of-sight,
  sort  = nlos,
  class = nomencl
}
\DeclareAcronym{PDR}{
  short = \normalfont{PDR} ,
  long  = Packet delivery ratio,
  sort  = pdr,
  class = nomencl
}
\DeclareAcronym{PSO}{
  short = \normalfont{PSO} ,
  long  = Particle swarm optimization,
  sort  = pso,
  class = nomencl
}
\DeclareAcronym{QL}{
  short = \normalfont{QL} ,
  long  = Q-learning,
  sort  = ql,
  class = nomencl
}
\DeclareAcronym{QoE}{
  short = \normalfont{QoE} ,
  long  = Quality of experience,
  sort  = qoe,
  class = nomencl
}
\DeclareAcronym{QoS}{
  short = \normalfont{QoS} ,
  long  = Quality of service,
  sort  = qos,
  class = nomencl
}

\DeclareAcronym{RAN}{
  short = \normalfont{RAN} ,
  long  = Radio access network,
  sort  = ran,
  class = nomencl
}

\DeclareAcronym{RL}{
  short = \normalfont{RL} ,
  long  = Reinforcement learning,
  sort  = rl,
  class = nomencl
}


\DeclareAcronym{SBS}{
  short = \normalfont{SBS} ,
  long  = Stationary base station,
  sort  = sbs,
  class = nomencl
}

\DeclareAcronym{TD}{
  short = \normalfont{TD} ,
  long  = Temporal difference,
  sort  = td,
  class = nomencl
}
\DeclareAcronym{TMFN}{
  short = \normalfont{TMFN} ,
  long  = Traffic-aware multi-tier flying network,
  sort  = tmfn,
  class = nomencl
}
\DeclareAcronym{UAV}{
  short = \normalfont{UAV} ,
  long  = Unmanned aerial vehicle,
  sort  = uav,
  class = nomencl
}

\DeclareAcronym{UAV-BS}{
  short = \normalfont{UAV-BS} ,
  long  = Unmanned aerial vehicles mounted base station,
  sort  = uav-bs,
  class = nomencl
}

\DeclareAcronym{UE}{
  short = \normalfont{UE} ,
  long  = User equipment,
  sort  = ue,
  class = nomencl
}

\DeclareAcronym{UTD}{
  short = \normalfont{UTD} ,
  long  = User traffic demand,
  sort  = utd,
  class = nomencl
}


==> nomenclature02.tex <==
\usepackage{acro}
\usepackage{enumitem}

\newlength\myitemwidth
\setlength\myitemwidth{5em} % <<< choose what you need here
\newlist{myacronymlist}{description}{1}
\setlist[myacronymlist]{
  labelindent = 0pt ,
  labelsep    = 0pt ,
  leftmargin  = \myitemwidth ,
  labelwidth  = \myitemwidth ,
  itemindent  = 0pt ,
  format      = \normalfont
}
%%%%%%%%%%%%%%
%\usepackage{acro}
% \DeclareAcroListStyle{myliststyle}{list}{
%   list = myacronymlist
% }
% \acsetup{ list-style = myliststyle }
%%%%%%%%%%%%%%%%

\NewAcroTemplate[list]{styleabbrev}{%
  \let\description\listabbrev
  \let\enddescription\endlistabbrev
  \UseAcroTemplate[list]{description}[0]%
}

\acsetup{
  list/template  = styleabbrev,
  list/heading   = chapter*,
  list/name      = Abkürzungen
}

\DeclareAcronym{UAV}{
  short = \normalfont{UAV} ,
  long  = Unmanned aerial vehicle,
  sort  = uav
}

\DeclareAcronym{EEG}{
  short = EEG,
  long  = Erneuerbare-Energien-Gesetz,
}

\DeclareAcronym{dbms}{
  short = DBMS,
  long  = Database Management System,
}

\DeclareAcronym{IoT}{
  short = \normalfont{IoT} ,
  long  = Internet-of-Things,
  sort  = i
}
\DeclareAcronym{4G}{
  short = \normalfont{4G} ,
  long  =  The fourth generation,
  sort  = 4
}
\DeclareAcronym{5G}{
  short = \normalfont{5G} ,
  long  =  The fifth generation,
  sort  = 5
}

\DeclareAcronym{6G}{
  short = \normalfont{6G} ,
  long  =  The sixth generation,
  sort  = 6
}

\DeclareAcronym{LDS}{
  short = \normalfont{LDS} ,
  long  =  Low-density spreading,
  sort  = lds
}

\DeclareAcronym{NOMA}{
  short = \normalfont{NOMA} ,
  long  =  Non-orthogonal multiple access,
  sort  = noma
}

\DeclareAcronym{MPA}{
  short = \normalfont{MPA} ,
  long  =  Message passing algorithm,
  sort  = mpa
}

\DeclareAcronym{MAP}{
  short = \normalfont{MAP} ,
  long  = Maximum a posteriori detector,
  sort  = map
}

\DeclareAcronym{MMSE}{
  short = \normalfont{MMSE} ,
  long  = Minimum mean-square estimation,
  sort  = mmse
}

\DeclareAcronym{BER}{
  short = \normalfont{BER} ,
  long  = Bit-error-rate,
  sort  = ber
}

\DeclareAcronym{MUD}{
  short = \normalfont{MUD} ,
  long  = Multiuser detection,
  sort  = mud
}


\DeclareAcronym{MIMO}{
  short = \normalfont{MIMO} ,
  long  = Multiple-input multiple-output,
  sort  = mimo
}

\DeclareAcronym{M2M}{
  short = \normalfont{M2M} ,
  long  = Machine-to-machine,
  sort  = m2m
}

\DeclareAcronym{D2D}{
  short = \normalfont{D2D} ,
  long  = Device-to-device,
  sort  = d2d
}

\DeclareAcronym{D2E}{
  short = \normalfont{D2E} ,
  long  = Device-to-everything ,
  sort  = d2e
}

\DeclareAcronym{IoV}{
  short = \normalfont{IoV} ,
  long  = Internet of Vehicles,
  sort  = iov
}

\DeclareAcronym{MTC}{
  short = \normalfont{MTC} ,
  long  = Machine-type communication,
  sort  = mtc
}

\DeclareAcronym{ITS}{
  short = \normalfont{ITS} ,
  long  = Intelligent transportation system,
  sort  = its
}

\DeclareAcronym{OMA}{
  short = \normalfont{OMA} ,
  long  = Orthogonal multiple access,
  sort  = oma
}

\DeclareAcronym{TDMA}{
  short = \normalfont{TDMA} ,
  long  = Time-division multiple access,
  sort  = tdma
}

\DeclareAcronym{FDMA}{
  short = \normalfont{FDMA} ,
  long  = Frequency division multiple access,
  sort  = fdma
}

\DeclareAcronym{CDMA}{
  short = \normalfont{CDMA} ,
  long  = Code-division multiple access,
  sort  = cdma
}


\DeclareAcronym{SCMA}{
  short = \normalfont{SCMA} ,
  long  = Sparse code multiple access,
  sort  = scma
}

\DeclareAcronym{PDMA}{
  short = \normalfont{PDMA} ,
  long  = Pattern division multiple access,
  sort  = pdma
}

\DeclareAcronym{MUSA}{
  short = \normalfont{MUSA} ,
  long  = Multiuser shared access,
  sort  = musa
}

\DeclareAcronym{MMTC}{
  short = \normalfont{mMTC} ,
  long  = Massive machine-type-communications,
  sort  = mmtc
}


\DeclareAcronym{LDPC}{
  short = \normalfont{LDPC} ,
  long  = Low-density parity-check,
  sort  = ldpc
}


\DeclareAcronym{AWGN}{
  short = \normalfont{AWGN} ,
  long  = Additive white Gaussian noise,
  sort  = awgn
}

\DeclareAcronym{FIR}{
  short = \normalfont{FIR} ,
  long  = Finite impulse response,
  sort  = fir
}

\DeclareAcronym{CIR}{
  short = \normalfont{CIR} ,
  long  = Channel impulse response,
  sort  = cir
}

\DeclareAcronym{MF}{
  short = \normalfont{MF} ,
  long  = Matched filter,
  sort  = mf
}

\DeclareAcronym{ZF}{
  short = \normalfont{ZF} ,
  long  = Zero-forcing filter,
  sort  = zf
}

\DeclareAcronym{SIC}{
  short = \normalfont{SIC} ,
  long  = Successive interference cancellation,
  sort  = sic
}

\DeclareAcronym{PIC}{
  short = \normalfont{PIC} ,
  long  = Parallel interference cancellation,
  sort  = pic
}

\DeclareAcronym{PDA}{
  short = \normalfont{PDA} ,
  long  = Probabilistic data association,
  sort  = pda
}

\DeclareAcronym{BP}{
  short = \normalfont{BP} ,
  long  = Believe propagation,
  sort  = bp
}

\DeclareAcronym{JSG}{
  short = \normalfont{JSG} ,
  long  = Joint sparse graph ,
  sort  = jsg
}



\iffalse
\DeclareAcronym{ML}{
  short = \normalfont{ML} ,
  long  = Maximum-likelihood,
  sort  = ml
}
\fi
\DeclareAcronym{FDE}{
  short = \normalfont{FDE} ,
  long  = Frequency domain equalization,
  sort  = fde
}

\DeclareAcronym{OFDM}{
  short = \normalfont{OFDM} ,
  long  = Orthogonal frequency-division multiplexing,
  sort  = ofdm
}

\DeclareAcronym{UD}{
  short = \normalfont{UD} ,
  long  = Uniquely decodable,
  sort  = ud
}

\DeclareAcronym{IrLDS}{
  short = \normalfont{IrLDS} ,
  long  = Irregular low-density spreading,
  sort  = irlds
}

\DeclareAcronym{VA}{
  short = \normalfont{VA} ,
  long  = Viterbi algorithm,
  sort  = va
}

\DeclareAcronym{SD}{
  short = \normalfont{SD} ,
  long  = Sphere-decoding algorithm,
  sort  = sd
}

\DeclareAcronym{SISO}{
  short = \normalfont{SISO} ,
  long  = Soft-input soft-output,
  sort  = siso
}

\DeclareAcronym{GML}{
  short = \normalfont{GML} ,
  long  = Global maximum likelihood detector,
  sort  = gml
}

\DeclareAcronym{SNR}{
  short = \normalfont{SNR} ,
  long  = Signal-to-noise ratio,
  sort  = snr
}

\DeclareAcronym{LRS}{
  short = \normalfont{LRS} ,
  long  = Large random spreading,
  sort  = lrs
}

\DeclareAcronym{QLSS}{
  short = \normalfont{QLSS} ,
  long  = Quasi-large sparse sequence,
  sort  = qlss
}

\DeclareAcronym{SER}{
  short = \normalfont{SER} ,
  long  = Symbol error rate,
  sort  = ser
}

\DeclareAcronym{MC}{
  short = \normalfont{MC} ,
  long  = Multicarrier,
  sort  = mc
}

\DeclareAcronym{JSFG}{
  short = \normalfont{JSFG} ,
  long  = Joint sparse factor graph,
  sort  = jsfg
}

\DeclareAcronym{SMI}{
  short = \normalfont{SMI} ,
  long  = Single user mutual information,
  sort  = smi
}

\DeclareAcronym{SVE}{
  short = \normalfont{SVE} ,
  long  = Spreading vector extension,
  sort  = sve
}

\DeclareAcronym{LDSM}{
  short = \normalfont{LDSM} ,
  long  = Low-density superposition modulation,
  sort  = ldsm
}

\DeclareAcronym{BBPSO}{
  short = \normalfont{BBPSO} ,
  long  = Bare-bone particle swarm optimization,
  sort  = bbpso
}

\DeclareAcronym{STS}{
  short = \normalfont{STS} ,
  long  = Steiner triple system,
  sort  = sts
}

\DeclareAcronym{BIBD}{
  short = \normalfont{BIBD} ,
  long  = Balanced incomplete block design,
  sort  = bibd
}

\DeclareAcronym{LDSMA}{
  short = \normalfont{LDSMA} ,
  long  = Low-density spreading multiple access,
  sort  = ldsma
}

\DeclareAcronym{GMAC}{
  short = \normalfont{GMAC} ,
  long  = Gaussian multiple access channel,
  sort  = gmac
}

\DeclareAcronym{BLER}{
  short = \normalfont{BLER} ,
  long  = Block error rate,
  sort  = bler
}

\DeclareAcronym{MAC}{
  short = \normalfont{MAC} ,
  long  = Multiple access channel,
  sort  = mac
}

\DeclareAcronym{EXIT}{
  short = \normalfont{EXIT} ,
  long  = Extrinsic information transfer,
  sort  = exit
}

\DeclareAcronym{SEP}{
  short = \normalfont{SEP} ,
  long  = Symbol error probability,
  sort  = sep
}

\DeclareAcronym{MS}{
  short = \normalfont{MS} ,
  long  = Mobile station,
  sort  = ms
}

\DeclareAcronym{SFBC}{
  short = \normalfont{SFBC} ,
  long  = Space-frequency block codes,
  sort  = sfbc
}

\DeclareAcronym{SM}{
  short = \normalfont{SM} ,
  long  = Spatial modulation,
  sort  = sm
}

\DeclareAcronym{SCDMA}{
  short = \normalfont{SCDMA} ,
  long  = Sparse code-division multiple-access,
  sort  = scdma
}

\DeclareAcronym{FBMC}{
  short = \normalfont{FBMC} ,
  long  = Filter-bank multicarrier,
  sort  = fbmc
}

% \DeclareAcronym{LDWM}{
%   short = \normalfont{LDWM} ,
%   long  = Low-density weight matrix,
%   sort  = ldwm
% }

% \DeclareAcronym{ULDS}{
%   short = \normalfont{ULDS} ,
%   long  = Ultra low-density spread,
%   sort  = ulds
% }

% \DeclareAcronym{SSM}{
%   short = \normalfont{SSM} ,
%   long  = Sparse superposition matrix,
%   sort  = ssm
% }

% \DeclareAcronym{SINR}{
%   short = \normalfont{SINR} ,
%   long  = Signal-to-interference-noise ratio,
%   sort  = sinr
% }

% \DeclareAcronym{TSC}{
%   short = \normalfont{TSC} ,
%   long  = Total squared correlation,
%   sort  = tsc
% }

% \DeclareAcronym{WBE}{
%   short = \normalfont{WBE} ,
%   long  = Welch-bound-equality,
%   sort  = wbe
% }

% \DeclareAcronym{MWBE}{
%   short = \normalfont{MWBE} ,
%   long  = Maximum-Welch-bound-equality,
%   sort  = mwbe
% }

% \DeclareAcronym{CM}{
%   short = \normalfont{CM} ,
%   long  = Coded modulation,
%   sort  = cm
% }

% \DeclareAcronym{MLCM}{
%   short = \normalfont{MLCM} ,
%   long  = Multilevel coded modulation,
%   sort  = mlcl
% }

% \DeclareAcronym{TCM}{
%   short = \normalfont{TCM} ,
%   long  = Trellis-coded modulation,
%   sort  = tcm
% }

% \DeclareAcronym{TTCM}{
%   short = \normalfont{TTCM} ,
%   long  = Turbo trellis-coded modulation,
%   sort  = ttcm
% }

% \DeclareAcronym{ED}{
%   short = \normalfont{ED} ,
%   long  = Euclidean distance,
%   sort  = ed
% }

% \DeclareAcronym{BICM}{
%   short = \normalfont{BICM} ,
%   long  = Bit-interleaved coded modulation,
%   sort  = bicm
% }

% \DeclareAcronym{LTE}{
%   short = \normalfont{LTE} ,
%   long  = Long-term evolution,
%   sort  = lte
% }

% \DeclareAcronym{QPP}{
%   short = \normalfont{QPP} ,
%   long  = Quadratic permutation polynomial,
%   sort  = qpp
% }

% \DeclareAcronym{PEG}{
%   short = \normalfont{PEG} ,
%   long  = Progressive edge-growth,
%   sort  = peg
% }

% \DeclareAcronym{EMB}{
%   short = \normalfont{EMB} ,
%   long  = Enhanced mobile broadband,
%   sort  = emb
% }

\DeclareAcronym{uRLLC}{
  short = \normalfont{uRLLC} ,
  long  = Ultra-reliable low-latency communications,
  sort  = urllc
}

\DeclareAcronym{mmWave}{
  short = \normalfont{mmWave} ,
  long  = Millimeter-wave,
  sort  = mmwave
}

\DeclareAcronym{AI}{
  short = \normalfont{AI} ,
  long  = Artificial intelligence,
  sort  = ai
}

\DeclareAcronym{BS}{
  short = \normalfont{BS} ,
  long  = Base station,
  sort  = bs
}

\DeclareAcronym{CNN}{
  short = \normalfont{CNN} ,
  long  = Convolutional neural network,
  sort  = cnn
}

\DeclareAcronym{DNN}{
  short = \normalfont{DNN} ,
  long  = Deep neural network,
  sort  = dnn
}

\DeclareAcronym{DQL}{
  short = \normalfont{DQL} ,
  long  = Deep Q-learning,
  sort  = dql
}

\DeclareAcronym{DQN}{
  short = \normalfont{DQN} ,
  long  = Deep Q-network,
  sort  = dqn
}

\DeclareAcronym{DRL}{
  short = \normalfont{DRL} ,
  long  = Deep reinforcement learning,
  sort  = drl
}

\DeclareAcronym{ER}{
  short = \normalfont{ER} ,
  long  = Experience replay,
  sort  = er
}

\DeclareAcronym{FMAP}{
  short = \normalfont{FMAP} ,
  long  = Flying mesh access point,
  sort  = fmap
}

\DeclareAcronym{GPS}{
  short = \normalfont{GPS} ,
  long  = Global positioning system,
  sort  = gps
}

\DeclareAcronym{LoS}{
  short = \normalfont{LoS} ,
  long  = Line-of-sight,
  sort  = los
}

\DeclareAcronym{ML}{
  short = \normalfont{ML} ,
  long  = Machine learning,
  sort  = ml
}
\DeclareAcronym{MDP}{
  short = \normalfont{MDP} ,
  long  = Markov decision process,
  sort  = mdp
}
\DeclareAcronym{MOS}{
  short = \normalfont{MOS} ,
  long  = Mean opinion score,
  sort  = mop
}
\DeclareAcronym{MINLP}{
  short = \normalfont{MINLP} ,
  long  = Mixed-integer non-linear problem,
  sort  = minlp
}

\DeclareAcronym{NLoS}{
  short = \normalfont{NLoS} ,
  long  = No-line-of-sight,
  sort  = nlos
}
\DeclareAcronym{PDR}{
  short = \normalfont{PDR} ,
  long  = Packet delivery ratio,
  sort  = pdr
}
\DeclareAcronym{PSO}{
  short = \normalfont{PSO} ,
  long  = Particle swarm optimization,
  sort  = pso
}
\DeclareAcronym{QL}{
  short = \normalfont{QL} ,
  long  = Q-learning,
  sort  = ql
}
\DeclareAcronym{QoE}{
  short = \normalfont{QoE} ,
  long  = Quality of experience,
  sort  = qoe
}
\DeclareAcronym{QoS}{
  short = \normalfont{QoS} ,
  long  = Quality of service,
  sort  = qos
}

\DeclareAcronym{RAN}{
  short = \normalfont{RAN} ,
  long  = Radio access network,
  sort  = ran
}

\DeclareAcronym{RL}{
  short = \normalfont{RL} ,
  long  = Reinforcement learning,
  sort  = rl
}


\DeclareAcronym{SBS}{
  short = \normalfont{SBS} ,
  long  = Stationary base station,
  sort  = sbs
}

\DeclareAcronym{TD}{
  short = \normalfont{TD} ,
  long  = Temporal difference,
  sort  = td
}
\DeclareAcronym{TMFN}{
  short = \normalfont{TMFN} ,
  long  = Traffic-aware multi-tier flying network,
  sort  = tmfn
}
% \DeclareAcronym{UAV}{
%   short = \normalfont{UAV} ,
%   long  = Unmanned aerial vehicle,
%   sort  = uav
% }

\DeclareAcronym{UAV-BS}{
  short = \normalfont{UAV-BS} ,
  long  = Unmanned aerial vehicles mounted base station,
  sort  = uav-bs
}

\DeclareAcronym{UE}{
  short = \normalfont{UE} ,
  long  = User equipment,
  sort  = ue
}

\DeclareAcronym{UTD}{
  short = \normalfont{UTD} ,
  long  = User traffic demand,
  sort  = utd
}

==> tables/neuron_changes_brant.tex <==
\begin{tabularx}{\textwidth}{|l|X|X|X|l|l|}
\hline
Neuron & User events covered by original neuron (circle in Figure \ref{fig:before_refinement}, inner circle in Figure \ref{fig:outer_radius} and orange circle in Figure \ref{fig:after_refinement}) & User events within \simeter{300} of original neuron (outer circle in Figure \ref{fig:outer_radius}) & User events covered by refined neuron (black points within blue circle in Figure \ref{fig:after_refinement}) & Increase & Percentage of increase\\
\hline
1 & 0 & 6 & 8 & 8 & $NaN$\\
\hline
2 & 86 & 212 & 181 & 95 & 110\%\\
\hline
\textbf{3} & 659 & 1118 & 819 & 160 & 24\%\\
\hline
4 & 106 & 190 & 122 & 16 & 15\%\\
\hline
\textbf{5} & 0 & 459 & 492 & 492 & $NaN$\\
\hline
\textbf{6} & 3220 & 5235 & 3292 & 72 & 2\%\\
\hline
\textbf{7} & 1618 & 3510 & 2199 & 581 & 36\%\\
\hline
8 & 333 & 575 & 384 & 51 & 15\%\\
\hline
9 & 381 & 635 & 418 & 37 & 10\%\\
\hline
10 & 199 & 410 & 307 & 108 & 54\%\\
\hline
\textbf{11} & 953 & 2173 & 1158 & 205 & 22\%\\
\hline
\textbf{12} & 311 & 645 & 508 & 197 & 63\%\\
\hline
\end{tabularx}

==> tables/task_sim.tex <==



==> tables/te_sim.tex <==
\begin{table*}[t]
 \caption{Simulation settings for task event generation. $\unif$ denotes a uniform distribution of a variable.}
    \centering
    \begin{tabularx}{\linewidth}{|L{.4}||L{1.3}|L{1.3}|}
        \hline
         & Malicious tasks & Legitimate tasks \\
        \hline
        Day & \multicolumn{2}{l|}{$\unif(\set{1, 2, \dots, 6})$} \\
        \hline
        Hour & $80\%$ from $\unif(\text{7:00}, \text{11:00})$; $20\%$ from $\unif(\text{12:00}, \text{17:00})$ & $\unif(\text{00:00}, \text{23:59})$ \\
        \hline
        Duration & $70\%$ from $\unif(\set{\simin{40}, \simin{50}, \simin{60}})$; $30\%$ from $\unif(\set{\simin{10}, \simin{20}, \simin{30}})$ & $\unif(\set{\simin{10}, \simin{20}, \dots, \simin{60}})$ \\
        \hline
        Smartphone battery usage & $50\%$ from $\unif(70\%, 10\%)$; $50\%$ from $\unif(1\%, 6\%)$ & $\unif(1\%, 10\%)$ \\
        \hline
        Coverage & \multicolumn{2}{l|}{$\simeter{100}$} \\
        \hline
        Movement radius & \multicolumn{2}{l|}{$\simeter{80}$} \\
        \hline
        % Number of days & $6$ \\
        % \hline
    \end{tabularx}
   
    \label{tab:te_sim}
\end{table*}


==> tables/ue_sim.tex <==
\begin{table}[!hbt]
\caption{Simulation settings for user event, attack center and task generation. $\unif$ denotes a uniform distribution of a variable.}
    \centering
    \begin{tabularx}{\linewidth}{|>{\hsize=.8\hsize\linewidth=\hsize}X|>{\hsize=1.2\hsize\linewidth=\hsize}X|}
        \hline
        Attack region radius ($R_a$) & $\SI{200}{\meter}$ \\
        \hline
        Number of users & $10000$ \\
        \hline
        Duration of user events & $\unif(\simin{60}, \simin{180})$ \\
        \hline
        Smartphone battery level & $80\%$\,from $\unif(20\%, 100\%)$; $20\%$ from $\unif(1\%, 20\%)$ \\
        \hline
        Sample rate of user events & $1 \text{ event/min}$ \\
        \hline
        Daily simulation time interval & 00:00 -- 23:59 \\
        \hline
        % Number of days & $6$ \\
        % \hline
        Number of attack centers & $6$ \\
        \hline
        Number of tasks & $\set{500, 1000, 2000}$ \\
        \hline
  
    \end{tabularx}
    
    \label{tab:ue_sim}
\end{table}

%\State $D$: Isolation constraint between neurons :400m
%    \State $R_{a}$: Attack range : 200m
%    \State $R$: Search region for neurons :200m (initial)
%    \State $R'$: Extended Search region for refinement: 300m

